Web Stereo Video Supervision for Depth Prediction from Dynamic Scenes

We present a fully data-driven method to compute depth from diverse monocular video sequences that contain large amounts of non-rigid objects, e.g., people. In order to learn reconstruction cues for non-rigid scenes, we introduce a new dataset consisting of stereo videos scraped in-the-wild. This dataset has a wide variety of scene types, and features large amounts of nonrigid objects, especially people. From this, we compute disparity maps to be used as supervision to train our approach. We propose a loss function that allows us to generate a depth prediction even with unknown camera intrinsics and stereo baselines in the dataset. We validate the use of large amounts of Internet video by evaluating our method on existing video datasets with depth supervision, including SINTEL, and KITTI, and show that our approach generalizes better to natural scenes.

==> sections/arap.tex <==

% \subsection{As-rigid-as-possible prior}
\subsection{cluster-wise ARAP (prior arts)}
Prior arts pose the as-rigid-as-possible (ARAP) prior at cluster level. That is, the template frame $\mathcal{T}$ is divided into $K$ clusters $\{\mathcal{S}_1, ..., \mathcal{S}_K\}$. First, each cluster $\mathcal{S}_k$ is assumed as a rigid object with individual motion $M_k$, which could be enforced by:
\begin{align}
    \mathcal{L}_\text{local} = \sum_k\sum_{i\in \mathcal{S}_k}\|M_k \begin{bmatrix}p_i \\ 1\end{bmatrix} 
    - p'_i\|
\end{align}
To glue each individual clusters together for a globally consistent 3D reconstruction , neighboring clusters are penalized to have similar rigid motion. One example of this is formulated as follow:
\begin{align}
    \mathcal{L}_\text{global} = \sum_{(k_1, k_2) \in E}\|M_{k_1} \begin{bmatrix}a_{k_1} \\ 1\end{bmatrix} - M_{k_2} \begin{bmatrix}a_{k_2} \\ 1 \end{bmatrix}\|, 
\end{align}
where $a_{k_1}$, $a_{k_2}$ denotes the 3D anchor points for two neighboring clusters.

The drawbacks for this cluster-wise ARAP approach are:
\begin{itemize}
    \item Dividing the whole image into non-overlapping strictly rigid moving clusters is not valid in real world.
    \item Requires explicitly solving the rigid motions $M_k$ in advance to evaluating the loss function. However, solving $M_k$'s with the presence of $\mathcal{L}_\text{global}$ is expensive and depends on iterative numerical algorithms. Moreover, it's laborious to implement $M_k$'s as a sub-differentiable function of the current depth estimation, which unfortunately is must-have for end-to-end training.
\end{itemize}


\subsection{pixel-wise ARAP (proposed)}
Primal goal of the proposed loss:
\begin{itemize}
    \item Each pixel is allowed to have individual rigid motion.
    \item Do not need to estimate rigid motions.
    \item Computationally efficient to evaluate.
\end{itemize}
To begin with, let's look at the local rigidity loss for pixel $i$ at an adaptive support region:
\begin{align*}
    \L^{(i)} = \sum_j w_{ij} \|M_i \begin{bmatrix}p_j\\1 \end{bmatrix} - p'_j\|^2,
\end{align*}
where $w_{ij}$ is the adaptive weights used to define the support region for pixel $i$. Ideally, nearby pixels with similar rigid motion as pixel $i$ should has higher weights; and distant pixels with different motion should has lower weights.

It turns out that if we allow to have reflection in $M_i$, then we don't need to know the exact value for $M_i$ to evaluate this loss, because:
\begin{align}
\label{eq:local_loss}
    \min_{M_i}\L^{(i)} = \sum_j w_{ij}\|\Tilde{p}_{ij}\|^2 - 2\| \sum_j w_{ij}\Tilde{p}_{ij}\Tilde{p'}_{ij}^T \|_\text{tr} + \sum_j w_{ij}\| \Tilde{p'}_{ij} \|^2,
\end{align}
where $\|\cdot\|_\text{tr}$ denotes trace (nuclear) norm, and
\begin{align}
    \label{eq:pt_norm}
    \Tilde{p}_{ij} = & p_j - \frac{\sum_{l} w_{il}p_l}{\sum_l w_{il}} \\
     \Tilde{p'}_{ij} = & p'_j - \frac{\sum_{l} w_{il}p'_l}{\sum_l w_{il}}
\end{align}

Although Eq.~\ref{eq:local_loss} get rid of $M_i$, naive implementation of this has a complexity of $O(m)$ if the support region has $m$ pixels, and the total cost of computation over an image with $n$ pixels is $O(mn)$. This renders it to be computationally too costly when the support region of a pixel is large. Fortunately, all the terms in Eq.~\ref{eq:local_loss},\ref{eq:pt_norm} can be implemented as bilateral filtering, and the most efficient variant of bilateral filtering, e.g. guided filter has a complexity of only $O(1)$ for each pixel.

Using guided filter not only allows us to use large support regions (e.g. $50\times50$), but also provides a good design for the adaptive filter weights $w_{ij}$, since it's edge aware.

\subsubsection{Dealing with occlusions}
We can have an occlusion mask $O$ by forward-backward flow consistency check. $o_i=0$ if pixel $i$ is occluded, and equals $1$ if otherwise. With the occlusion mask, Eq.~\ref{eq:local_loss} is modified as:
\begin{align}
    \L^{(i)} = & \sum_j w_{ij}o_j\|\Tilde{p}_{ij}\|^2 - 2\| \sum_j w_{ij}o_j\Tilde{p}_{ij}\Tilde{p'}_{ij}^T \|_\text{tr} \\
    & + \sum_j w_{ij}o_j\| \Tilde{p'}_{ij} \|^2,
\end{align}
And it still can be efficiently implemented by guided fliter.

\subsubsection{Implementation via guided filtering}
Denote $\mathcal{F}(\cdot)$ as guided filtering with some guidance image, and it's  output at pixel $i$ is represented as $\mathcal{F}_i(\cdot)$.
\begin{align*}
    \Bar{\bold{p}}_i = \frac{\sum_{j} w_{ij} (o_j \bold{p}_j)}{\sum_j w_{ij} o_j} = \frac{[\mathcal{F}_i(\bold{O}\circ\bold{P_x}), \mathcal{F}_i(\bold{O}\circ\bold{P_y}), \mathcal{F}_i(\bold{O}\circ\bold{P_z})]^T}{\mathcal{F}_i(\bold{O})}
\end{align*}

\begin{align*}
   & \sum_j w_{ij} o_j \|\Tilde{\bold{p}}_{ij}\|^2 \\
   = & \sum_j w_{ij}o_j \|\bold{p}_j - \Bar{\bold{p}}_i\|^2 \\
   = & \sum_j w_{ij} o_j \|\bold{p}_j\|^2 -2\Bar{\bold{p}}_i^T\sum_j w_{ij}o_j  \bold{p}_j + (\sum_j w_{ij}o_j)\|\Bar{\bold{p}}_i\|^2
\end{align*}


\begin{align*}
   & \sum_j w_{ij}o_j\Bar{\bold{p}}_{ij} \Bar{\bold{p}'}_{ij}^T \\
   = & \sum_j w_{ij} o_j (\bold{p}_{j}-\Bar{\bold{p}}_i)(\bold{p}_{j}'-\Bar{\bold{p}}'_i)^T \\
   = & \sum_j w_{ij} o_j \bold{p}_j\bold{p}_j'^T
   - (\sum_j w_{ij}o_j \bold{p}_j) \Bar{\bold{p}}_i'^T - \Bar{\bold{p}}_i (\sum_j w_{ij}o_j \bold{p}_j')^T + (\sum_j w_{ij}o_j) \Bar{\bold{p}}_i\Bar{\bold{p}}_i'^T
\end{align*}







==> sections/includes.tex <==
\usepackage{url}
\usepackage{amsthm}
\usepackage{color}
\usepackage{subcaption}
\captionsetup{compatibility=false}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{pbox}
\usepackage[demo,abs]{overpic}
\usepackage{enumitem}


\usepackage{colortbl}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{tablefootnote}
\usepackage{tabularx}
\definecolor{rowblue}{RGB}{220,230,240}

%%% From https://tex.stackexchange.com/questions/1522/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink.
%href fix
\usepackage{etoolbox}
\makeatletter
\patchcmd\@combinedblfloats{\box\@outputbox}{\unvbox\@outputbox}{}{\errmessage{\noexpand patch failed}}
\makeatother
%%%
\newcommand{\fp}[1]{\textbf{\textcolor[rgb]{.1, .1, .8}{FP: #1}}}
\newcommand{\ow}[1]{\textbf{\textcolor[rgb]{.1, .8, .1}{OW: #1}}}
\newcommand{\cy}[1]{\textbf{\textcolor[rgb]{.8, .1, .1}{CY: #1}}}
\newcommand{\todo}[1]{\textbf{\textcolor[rgb]{.8, .2, .1}{#1}}}

\newcommand{\dataset}{\textsc{WSVD}}
\newcommand{\network}{\textsc{2-view depth net}}

% space hack
\setlength{\belowcaptionskip}{-5pt}


==> sections/report.tex <==
% \begin{align}
% \mathbf{x}'= &\mathcal{W}(\mathbf{x}; d,\alpha, \beta)\\
% = & \begin{bmatrix}x-\alpha d+\beta\\
% y \end{bmatrix}
% \end{align}

% where $\alpha = fb$, $\beta = c_x - c'_x$.

% $\alpha$ and $\beta$ is unknown for 3D movies collected from the Internet.

% Training objective:
% \begin{equation}
%     \min_{\theta,\alpha>0,\beta} \L_\text{photo}\bigg(\I_\text{L}, \I_\text{R}\left(\W\left(\cdot;\mathbf{d}_\theta, \alpha, \beta\right)\right)\bigg) + \L_\text{grad}(\mathbf{d}_\theta, \mathbf{d}^*)
% \end{equation}
\section{Primaries}

\subsection{Camera intrinsics}
Assumes the cameras are rectified.
$$\mathbf{K}_\text{left}=\begin{bmatrix}
      f & 0 & c_u+\frac{1}{2}d_\text{min}\\
      0 & \alpha f & c_v\\
      0 & 0 & 1
    \end{bmatrix}$$

$$\mathbf{K}_\text{right}=\begin{bmatrix}
      f & 0 & c_u-\frac{1}{2}d_\text{min}\\
      0 & \alpha f & c_v\\
      0 & 0 & 1
    \end{bmatrix}$$

where $\alpha$ is the aspect ratio(assume it's given); $(c_u,c_v)$ is the coordinate of image center; $d_\text{min}$ denotes the minimum disparity.

\subsection{Projection between stereo temporal pairs}
The projection of a point $\p^t_l=(u,v)^T$ in $I_\text{left}^{t}$ to $I_\text{left}^{t+1}$ is computed as:
$$\begin{bmatrix}\Tilde{\p}_l^{t+1}\\1\end{bmatrix}=\mathbf{K}_\text{left}\left<
\R \mathbf{K}^{-1}_\text{l
eft}\begin{bmatrix}\p^t_l\\1\end{bmatrix} +\frac{d-d_\text{min}}{bf} \t 
\right>$$
here, $b$ is baseline of the stereo rig, and $d$ denotes disparity. $<\cdot>$ denotes projection:
$$<[x,y,z]^T> = [x/z, y/z, 1]^T$$

Since both $b$ and $\t$ are up-to-scale, we could directly parameterize $\frac{\t}{b}$ by $\Tilde{\t}$ with only 3 D0F:
$$\Tilde{\t} = \frac{\t}{f}$$

\subsection{Bundle adjustment}
\label{sec:ba}
Given correspondences between stereo temporal pairs, estimate $f$,$d_\text{min}$,$\R$, $\Tilde{\t}$  by minimizing the reprojection error:
$$\L_\text{repro}=h(\Tilde{\p}_l^{t+1}-\p_l^{t+1})$$
here $h$ can be ssd, huber or other robust loss functions.
This can be solved via Gauss-Newton method.

\section{Create ``ground truth''}
\subsection{compute optical flow by PWC-net}
compute optical flow between stereo pairs, temporal pairs, and also stereo temporal pairs, e.g. $\I_\text{left}^t\longleftrightarrow\I_\text{right}^{t+1}$
\subsection{filter optical flow}
 filter optical flow results through forward backward consistency check, retain correspondences which are consistent across all the pairs.
 
 If the remaining correspondences are lower than certain percentage, discard the whole data point, since it's likely a failure case for the flow estimation algorithm.
\subsection{camera calibration and bundle adjustment}
run Ransac with 8 point algorithm to select candidate correspondences belonging to the background.
perform bundle adjustment described in sec.~\ref{sec:ba}

\subsection{label motion segmentation}
identify moving pixels by reprojection error

\section{Learning with ``ground truth''}
\subsection{Learning to predict motion segmentation}
\subsection{Learning to predict scene flow}
\subsection{Learning to predict depth}

\section{Combining photometric loss}
\subsection{stereo camera}
\subsection{single camera}



